FPRaker: A Processing Element For Accelerating Neural Network Training

We present FPRaker, a processing element for composing training accelerators. FPRaker processes several floating-point multiply-accumulation operations concurrently and accumulates their result into a higher precision accumulator. FPRaker boosts performance and energy efficiency during training by taking advantage of the values that naturally appear during training. Specifically, it processes the significand of the operands of each multiply-accumulate as a series of signed powers of two. The conversion to this form is done on-the-fly. This exposes ineffectual work that can be skipped: values when encoded have few terms and some of them can be discarded as they would fall outside the range of the accumulator given the limited precision of floating-point. We demonstrate that FPRaker can be used to compose an accelerator for training and that it can improve performance and energy efficiency compared to using conventional floating-point units under ISO-compute area constraints. We also demonstrate that FPRaker delivers additional benefits when training incorporates pruning and quantization. Finally, we show that FPRaker naturally amplifies performance with training methods that use a different precision per layer.

==> scraps.tex <==
\begin{comment}
which motivates splitting the shifting into two stages as:

\begin{figure}[ht]
    \begin{minipage}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.24]{figs/Pragmatic_s2_shift.png} 
    \label{fig:PRA_s2_shift_eq}
    \end{minipage}
\end{figure}

Thus, to shift and add 8 weights by different offsets $K_0,...,K_7$, we can decompose the offsets into sums with a common term $C$. This has the advantage of reducing the area of alignment shifters and adder tree by sharing one common shifter after the adder tree with little to no performance overhead. 

%Fig. \ref{fig:FP_PRA_s2_shift} gives an example of the operation of the 2-stage shifting. By restricting the size of the alignment shifters using a design parameter $L$, the design can only process offsets less than $2^{L}$ in a single cycle.
\end{comment}




\begin{comment}
\begin{equation} \label{PRA_eq}
\begin{split}
(2^{A_{e}}\times A_s) \times (2^{B_e}\times B_s) = 2^{A_{e}+B_{e}} \times \sum_{i=0}^{p}A_s^{i} . (B_s\ll i)
\end{split}
\end{equation}

\begin{equation} \label{PRA_eq}
\begin{split}
(2^{A_{e}}\times A_s) \times (2^{B_e}\times B_s) + (2^{C_{e}}\times C_s) \times (2^{D_e}\times D_s)\\ = 2^{A_{e}+B_{e}} \times(\sum_{i=0}^{p}A_s^{i} . (B_s\ll i) + \sum_{j=0}^{p}C_s^{j} . (D_s\ll j+\delta))\\
\delta = (A_{e}+B_{e})-(C_{e}+D_{e})
\end{split}
\end{equation}


To exploit bit-sparsity of one of its operands, Pragmatic decomposes the multiplication operation into a series of "Shift and Add" operations. Eq. \ref{PRA_eq} shows such decomposition in floating-point, where $A_s$ and $W_s$ stands for activation and weight significand respectively. 

Pragmatic achieves performance speedups and energy efficiency by processing only the effectual bits (we refer to their positions as "terms") in the activation significand.

As mentioned earlier, a modified Pragmatic PE that targets floating-point operations is useful to accelerate DNN training and inference of some NLP models. For NLP inference, either the side of activations or weights can be serialized depending on the operand with the highest bit-sparsity. The modified Pragmatic will exploit the activation bit-sparsity in eq. \ref{forward_eq}, and the output gradient and input activation bit-sparsity in eq. \ref{backward_eq1} and eq. \ref{backward_eq2} respectively. Fig. \ref{fig:processed_bits_PRA} shows the average number of processed bits in the multiply operations by Pragmatic PE weighted with the number of multiply operations per layer. 

\begin{figure}[ht]
    \begin{minipage}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.27]{figs/avg_processed_bits_BF16_Pragmatic.png} 
    \caption{Weighted average of the number of processed bits in 8bx8b multiplication (Bfloat16). Lower is better.}
    \label{fig:processed_bits_PRA}
    \end{minipage}
\end{figure}



\begin{figure*}[h!]
    \begin{minipage}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.85]{figs/FP_Pragmatic_new_s2_shift.png} 
    \caption{\small{Modified Pragmatic 2-stage shifting. Example: Processing 2 activation and weight pairs with $L = 4$. Each cycle, the offset generators reads two final offsets produced in the step 1. The minimum offset controls the second stage shifter. The control subtracts the offsets from the minimum and sends the difference to the first stage shifters as long as they are less than $2^{L}$. In cycle 0, the control reads offsets (0,4), selects 0 to be sent to the seconds stage shifter, and sends 0 and 4 to the first stage shifter. In cycle 2, it reads offsets (8,15), sends 8 to seconds stage shifter, and sends 0 and 7 to first stage shifters. In cycle 3, it reads only one offset (21). Since the offset is larger than $2^{L}$, it sends 15 to the upper first stage shifters and 6 to the second stage shifter, while the lower first stage shifter is disabled. Unfortunately, unlike Pragmatic, since the offset generators reads the final product terms (includes activation and weight exponents), they cannot be shared across multiple PEs.}}
    \label{fig:FP_PRA_s2_shift}
    \end{minipage}
\end{figure*}
\end{comment}



\begin{comment}
\ssubsection{Base-Delta Exponent Compression}\label{base_delta_compression}
As shown earlier in fig. \ref{fig:exp_resnet34}, the exponents of input activations, weights, and output gradients lie within a narrow range. Hence, this observation can be used to reduce the memory requirements during training, as well as reducing the datapath of block (1) in fig. \ref{fig:FP_PRA_intial} through a compression scheme such as base-delta compression.

\begin{figure}[ht]
    \begin{minipage}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.32]{figs/expon} 
    \caption{Average required bit-width for delta exponents using base-delta compression on models trained on ImageNet}
    \label{fig:baseDelta_bits}
    \end{minipage}
\end{figure}

Fig. \ref{fig:baseDelta_bits} shows the required bit-width by the exponent deltas within groups of 32 parameters. For most networks, supporting 8-bits for exponents is overprovisioning, and 4-bit exponents are enough. For cases that require more than 4-bits, the exponent can be decomposed into multiple smaller exponents to be processed within 4-bits in multiple cycles.
\end{comment}
